Automatic Labelling with Open-source LLMs using Dynamic Label Schema Integration

Acquiring labelled training data remains a costly task in real world machine learning projects to meet quantity and quality requirements. Recently Large Language Models (LLMs), notably GPT-4, have shown great promises in labelling data with high accuracy. However, privacy and cost concerns prevent the ubiquitous use of GPT-4. In this work, we explore effectively leveraging open-source models for automatic labelling. We identify integrating label schema as a promising technology but found that naively using the label description for classification leads to poor performance on high cardinality tasks. To address this, we propose Retrieval Augmented Classification (RAC) for which LLM performs inferences for one label at a time using corresponding label schema; we start with the most related label and iterates until a label is chosen by the LLM. We show that our method, which dynamically integrates label description, leads to performance improvements in labelling tasks. We further show that by focusing only on the most promising labels, RAC can trade off between label quality and coverage - a property we leverage to automatically label our internal datasets.

==> comments.tex <==

% Story line comments
- contribution of the paper is unclear:
    - unclear what prompt changes were made (Table 5) 
    - RAC contribution  / effect is unclear (why did the authors examine the MRR in Table 3) (add time improvement?) 
    - industry motivation (creation of high quality labelling, public LLM, internal dataset, etc) 
- which category? emerging or discovery? --> needs to be clear in the narrative

% discussion what what should be the contribution
- open source, liscence to deploy internally --> see at current stage if they are able to provide what API based models such as ChatGPT, etc. using LLM that complies with privacy, etc. 
    - other works on this angle: prompting llms for data annotation (weak supervision) 
    - LLM for classification
- RAC --> retrieving instructions for classification. 
    - why is it novel
    - RAC turns binary into a multi-class task --> 
- take out multi-agent framework

% Experimentation:
- any internal dataset experiments we should run?
- RAC time experiments?

% Writing suggestions:
- Line 023: “multi-agent framework, etc.” This line is unclear until figure 2 and not sure it is a major contribution. 
- line 005: “evolving label schema, etc.” I was expecting the authors to discuss these but I don’t see it further down the paper. Please remove information irrelevant to the paper (even if they are interesting and related).
- line 066: “leading to costs that scale, etc.” Similarly, I expected materials down the line but there is no such materials further. 
- Ziems 2023 and Reiss 2023 seem indeed related, and it would be better if authors could explain how they come to such suggestions/conclusions.
- line 151 states the focus of this work but it is in related work section and not so much in abstract and introduction. 
- The methodology and experiment settings are a bit mixed altogether: e.g. line 173-175, and vllm line 178-200 are clearly experimental settings. 
- 3.4 RAC seems worth further details and being clarified in writings. It is curious to see so little in methods but so much in results for this part. 
- For all D and L+D experiments, the authors should share prompts for reviewing and examinations.


% Chunyang comments
At high level, I would say that the paper contains enough content to be potentially accepted at industry track. However, I can’t see the clear contribution of the paper after reading it. My other confusion point is that I thought the paper would be in emerging category but the paper more reads like discovery category https://2024.naacl.org/calls/industry/. Below are my details comments:

Pros:
The paper studies through several public benchmarks how to create annotated data by using public small LLMs. Based on current SOTA methods, the paper leverages label schema, self consistency and an admistrative pipeline to improve the labelling accuracy. The authors seem to show the utility of such auto-labels in Table 4 where 1) the performance of the overall pipeline sometimes match the training accuracy 2) one can further perform distillation where the accuracy remains similar. 

Cons: 
The contribution of the paper is unclear after my reading. The paper claims 3 contributions: label schema information, self consistency and the administrative pipeline. As clarified by the paper itself, label schema information and self consistency are based on current SOTA methods and while Table 5 shows improved results with the administrative pipeline, one does not know the process and the exact prompt changes after reading the paper and I am not sure if it consists itself a widely applicable pipeline for general industry. At the same time, there seems to be other innovations happening inside this project (RAC, public small LLMs) that are not very clear and not put forward by the authors. 

The other unclear part related to above is that I don’t see the industry motivation behind the paper. While creating data is always useful, apart from using public LLM that I can deduce, it is not sure what the authors want to achieve for the corresponding enterprise through the experiments, maybe creating high quality labelling? It would be great that the authors clarify themselves through the paper. The authors don’t mention about the motivation neither their internal datasets at all throughout the paper. 

My final confusion point is the RAC part. It seems to be some innovation that authors don’t want to put forward and the techniques seem unclear to me: for example, why did the authors examine the MRR in Table 3 (which takes a lot of place by the way).
 
Writing suggestions:
As I clarified previously, I believe the paper would benefit from a more careful storytelling clarifying motivation, innovation and conclusions/insights. Below are some minor writing suggestions:
- Line 023: “multi-agent framework, etc.” This line is unclear until figure 2 and not sure it is a major contribution. 
- line 005: “evolving label schema, etc.” I was expecting the authors to discuss these but I don’t see it further down the paper. Please remove information irrelevant to the paper (even if they are interesting and related).
- line 066: “leading to costs that scale, etc.” Similarly, I expected materials down the line but there is no such materials further. 
- Ziems 2023 and Reiss 2023 seem indeed related, and it would be better if authors could explain how they come to such suggestions/conclusions.
- line 151 states the focus of this work but it is in related work section and not so much in abstract and introduction. 
- The methodology and experiment settings are a bit mixed altogether: e.g. line 173-175, and vllm line 178-200 are clearly experimental settings. 
- 3.4 RAC seems worth further details and being clarified in writings. It is curious to see so little in methods but so much in results for this part. 
- For all D and L+D experiments, the authors should share prompts for reviewing and examinations.
 
Thank you
 
PS: Please advise if I should get further involved in the project. As detailed above, I think the paper would benefit from a careful storytelling and writing improvement, which I could help if people agree and want to push further down the line and of course, this needs a bit planning, discussing and concrete writing iterations. That being said, I agree that even at this stage, the paper still has some chance to be accepted, the disparity between pros and cons is intentional �� so that we can potentially improve ��  


% sally TODO:
- upload all prompts
- run baseline (1 shot classification) on b77, time and performance
- run banking all again for performance
- create whatsapp group
- create meeting on friday
- upload internal dataset results from internship presentation


experiments (time, performance) 
- FullRAC
- FullRAC + random index (baseline)
- multiclass classification with single prompt

